Determination of $\alpha_{S}$ beyond $NNLO$ using the event shape averages

In this proceedings we discuss a prescription to extract the QCD strong coupling constant at $N^{3}LO$ precision in perturbative QCD using a combination of ${\cal{O}}(\alpha_{S}^{3})$ calculations in pQCD and estimations of the ${\cal{O}}(\alpha_{S}^{4})$ corrections from the data. The method is applied to a set of event shape averages measured in experiments at the LEP, PETRA, PEP and TRISTAN colliders. In our analysis we account for hadronization effects with models from modern Monte Carlo event generators and analytic hadronization models. We conclude that the precision of the $\alpha_{S}$ extraction cannot be improved significantly only with pQCD predictions of higher orders, and further progress in these studies requires a significant advances in the studies and modeling of hadronization process.

==> Makefile <==
#ulimit -u 10000
latexfile?=MOM
newname?=MOM
STYLE=proceedings




LATEX=  lualatex -halt-on-error -shell-escape -enable-write18
LATEX=  pdflatex -halt-on-error -shell-escape -enable-write18
BIBTEX=bibtex



latexfiles= $(latexfile)-def.tex $(latexfile)-txt.tex $(latexfile)-val.tex 
ifeq ($(STYLE),proceedings)
	latexfiles=
	STYLE_SPECIFIC_FILES=$(latexfile)-proceedings.tex $(latexfile)-val.tex $(latexfile)-def.tex  SciPost.cls SciPost_bibstyle.bst ismd-logo-rect.png 
endif


ifeq ($(STYLE),draft)
	STYLE_SPECIFIC_FILES=zeus_paper.cls $(latexfile)-draft.tex $(latexfile).bst
endif

ifeq ($(STYLE),arxiv)
	STYLE_SPECIFIC_FILES=zeus_paper.cls $(latexfile)-arxiv.tex $(latexfile).bst
endif

ifeq ($(STYLE),epjc)
	STYLE_SPECIFIC_FILES=svjour.cls  svepj.clo $(latexfile)-epjc.tex $(latexfile).bst
endif


all: $(latexfile)-$(STYLE).pdf

tar:  Makefile $(figures) $(constanttables) $(tables)   $(latexfiles) $(STYLE_SPECIFIC_FILES)
	rm -rf TAR
	mkdir -p TAR
	cp Makefile   $(latexfiles)  $(latexfile).bib   $(STYLE_SPECIFIC_FILES) TAR
ifeq ($(STYLE),epjc)
	cp $(figures) TAR/
else
	mkdir -p TAR/Figures
	cp $(figures) TAR/Figures
endif
	sed -i 's@'$(latexfile)'@'$(newname)'@g' TAR/*tex	
	sed -i 's@'$(latexfile)'@'$(newname)'@g' TAR/Makefile
	sed -i 's@^STYLE.*@STYLE='$(STYLE)'@g' TAR/Makefile
	sed -i '/@artic/achecked={2},'     TAR/*bib	
	sed -i '/@inproceed/achecked={2},' TAR/*bib	
	sed -i '/@phdthesis/achecked={2},' TAR/*bib	

ifeq ($(STYLE),epjc)
	sed -i 's@\[htbp\]@@g' TAR/$(latexfile)-tab.tex
	sed -i 's@c|@c@g' TAR/$(latexfile)-tab.tex
	sed -i 's@|c@c@g' TAR/$(latexfile)-tab.tex
	sed -i 's@}|@}@g' TAR/$(latexfile)-tab.tex
endif

ifneq ($(STYLE),proceedings)
	mv TAR/$(latexfile).bst TAR/$(newname).bst 
endif
	mv TAR/$(latexfile).bib TAR/$(newname).bib 
	mv TAR/$(latexfile)-$(STYLE).tex TAR/$(newname)-$(STYLE).tex
ifeq ($(STYLE),epjc)
	sed -i 's@Figures/@@g' TAR/Makefile
endif
ifeq ($(STYLE),proceedings)
	mv TAR/$(latexfile)-def.tex TAR/$(newname)-def.tex
	cat TAR/$(latexfile)-val.tex | grep [:0-9:] > TAR/$(newname)-val.tex
	rm -f TAR/$(latexfile)-val.tex TAR/$(newname)-txt.tex TAR/$(latexfile).bst TAR/$(newname).bst 
	$(MAKE) -C TAR
	mv TAR/$(newname)-$(STYLE).bbl  TAR/$(newname)-$(STYLE).bbl.temp
	$(MAKE) -C TAR clean
	mv TAR/$(newname)-$(STYLE).bbl.temp  TAR/$(newname)-$(STYLE).bbl
	rm -rf TAR/$(newname).bib 
endif
ifeq ($(STYLE),arxiv)
	#####-->A trick to get the bib file for axiv build system
	$(MAKE) -C TAR
	mv TAR/$(newname)-$(STYLE).bbl  TAR/$(newname)-$(STYLE).bbl.temp
	$(MAKE) -C TAR clean
	mv TAR/$(newname)-$(STYLE).bbl.temp  TAR/$(newname)-$(STYLE).bbl
endif
ifeq ($(STYLE),epjc)
	#####-->A trick to get the bib file for axiv build system
	$(MAKE) -C TAR
	mv TAR/$(newname)-$(STYLE).bbl  TAR/$(newname)-$(STYLE).bbl.temp
	$(MAKE) -C TAR clean
	mv TAR/$(newname)-$(STYLE).bbl.temp  TAR/$(newname)-$(STYLE).bbl
endif
	tar -zcvf   $(newname).tar.gz -C TAR . 
	rm -rf $(newname).zip; cd TAR; zip ../$(newname).zip ./*/* ./*; cd ..

	rm -rf TAR


figures=  Figures/figC1-figure0.pdf      \
           Figures/fighadC1-figure0.pdf     \
           Figures/fighadoneminusT1-figure0.pdf   \
           Figures/figoneminusT1-figure0.pdf   
tables=
constanttables=


$(latexfile)-$(STYLE).pdf :  $(figures) $(constanttables) $(tables) \
                    $(latexfiles)  $(latexfile).bib  $(STYLE_SPECIFIC_FILES)
	$(LATEX) $(latexfile)-$(STYLE)
	$(LATEX) $(latexfile)-$(STYLE)
	$(BIBTEX) $(latexfile)-$(STYLE)
	$(BIBTEX) $(latexfile)-$(STYLE)
ifeq ($(STYLE),epjc)
	sed -i 's@\\mbox{}.*@@g'  $(latexfile)-$(STYLE).bbl
endif
ifeq ($(STYLE),arxiv)
	sed -i 's@\\mbox{}.*@@g'  $(latexfile)-$(STYLE).bbl
endif
	sed -i 's@Collaboration@Coll\.@g'  $(latexfile)-$(STYLE).bbl
	$(LATEX) $(latexfile)-$(STYLE)
	$(LATEX) $(latexfile)-$(STYLE)

pdf : $(latexfile)-$(STYLE).pdf

$(latexfile).rws: $(latexfile)-dict.txt
	aspell --lang=en create master ./$(latexfile).rws < ./$(latexfile)-dict.txt

spell: $(latexfile).rws
	for a in $$(ls -1 $(latexfile)-*.tex ); do\
		echo "%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%" ;\
		echo $a;\
		echo "%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%" ;\
		aspell  --add-extra-dicts=./$(latexfile).rws  -t --dont-tex-check-comments -d en_GB -c $$a ;\
	done

clean :
	rm -f *.aux
	rm -f *.lof
	rm -f *.out
	rm -f *.lot
	rm -f *.bbl
	rm -f *.l4l
	rm -f *.log
	rm -f *.blg
	rm -f *.ilg
	rm -f *.aux
	rm -f $(latexfile)*.dvi
	rm -f $(latexfile)*.ps
	rm -f $(latexfile)*.pdf
	rm -f *.toc
	rm -f *.idx
	rm -f *.ind
	rm -f *.nav
	rm -f *.snm


